HyGEN: Regularizing Negative Hyperedge Generation for Accurate Hyperedge Prediction

Hyperedge prediction is a fundamental task to predict future high-order relations based on the observed network structure. Existing hyperedge prediction methods, however, suffer from the data sparsity problem. To alleviate this problem, negative sampling methods can be used, which leverage non-existing hyperedges as contrastive information for model training. However, the following important challenges have been rarely studied: (C1) lack of guidance for generating negatives and (C2) possibility of producing false negatives. To address them, we propose a novel hyperedge prediction method, HyGEN, that employs (1) a negative hyperedge generator that employs positive hyperedges as a guidance to generate more realistic ones and (2) a regularization term that prevents the generated hyperedges from being false negatives. Extensive experiments on six real-world hypergraphs reveal that HyGEN consistently outperforms four state-of-the-art hyperedge prediction methods.

==> tables/datasets.tex <==
\begin{table*}[t]
\centering

\caption{Statistics of datasets used in our experiments.}\label{table:datasets}
\setlength\tabcolsep{6pt} % column space
\def\arraystretch{1.0} % row space

\begin{tabular}{c|rrc}
\toprule

Name & \# of Nodes & \# of Edges & Domain \\ 

\midrule
Citeseer & 1,457 & 1,078 & Co-citation \\ 
Cora & 1,434 & 1,579 & Co-citation \\ 
Pubmed & 3,840 & 7,962 & Co-citation \\ 
Cora-A & 2,388 & 1,072 & Authorship \\ 
DBLP-A & 39,283 & 16,483 & Authorship \\ 
DBLP & 15,639 & 22,964 & Collaboration \\ 

\bottomrule
\end{tabular}
\end{table*}


==> tables/eq1-accuracy.tex <==
\begin{table*}[t]
\centering
\caption{Hyperedge prediction accuracy on six hypergraphs. {\method} consistently outperforms all competitors in terms of both AUROC and AP averaged. For each dataset, the best and the second-best results are highlighted in the \textbf{bold} font and \underline{underlined}, respectively. OOM indicates out of memory' on a 11GB GPU.}\label{table:eval-accuracy}
\setlength\tabcolsep{3.3pt} % column space
\def\arraystretch{1.0} % row space
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}crrrrrrrr|rrrrrrrr@{}}

\toprule

\multicolumn{1}{c|}{Dataset} & \multicolumn{8}{c|}{Citeseer} & \multicolumn{8}{c}{Pubmed} \\ 
\midrule
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c|}{\scriptsize AP} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c}{\scriptsize AP} \\ 
\midrule
\multicolumn{1}{c|}{Test set} & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG \\ 
\midrule
\midrule
\multicolumn{1}{c|}{Expansion} & 0.663 & 0.781 & 0.331 & \multicolumn{1}{c|}{0.592} & 0.765 & 0.817 & 0.498 & 0.693 & 0.520 & 0.730 & 0.241 & \multicolumn{1}{c|}{0.497} & 0.675 & 0.755 & 0.440 & 0.623 \\
\multicolumn{1}{c|}{NHP} & {\color[HTML]{0000FF} 0.991} & 0.701 & 0.510 & \multicolumn{1}{c|}{0.734} & {\color[HTML]{0000FF} 0.990} & 0.731 & 0.520 & 0.747 & {\color[HTML]{0000FF} 0.973} & 0.694 & 0.524 & \multicolumn{1}{c|}{0.730} & {\color[HTML]{0000FF} 0.973} & 0.656 & 0.513 & 0.714 \\
\multicolumn{1}{c|}{HyperSAGNN} & 0.540 & 0.410 & 0.473 & \multicolumn{1}{c|}{0.474} & 0.627 & 0.455 & 0.497 & 0.526 & 0.525 & 0.686 & {\color[HTML]{0000FF} 0.546} & \multicolumn{1}{c|}{0.586} & 0.534 & 0.680 & {\underline{0.529}} & 0.581 \\
\multicolumn{1}{c|}{AHP} & 0.943 & {\underline{0.881}} & {\underline{0.651}} & \multicolumn{1}{c|}{{\underline{0.825}}} & 0.952 & {\underline{0.870}} & {\underline{0.660}} & {\underline{0.827}} & 0.917 & {\underline{0.840}} & {\underline{0.533}} & \multicolumn{1}{c|}{{\underline{0.763}}} & 0.918 & {\underline{0.834}} & 0.526 & {\underline{0.759}} \\
\multicolumn{1}{c|}{{\method}} & {\underline{0.984}} & {\color[HTML]{0000FF} 0.926} & {\color[HTML]{0000FF} 0.676} & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.862}} & {\underline{0.985}} & {\color[HTML]{0000FF} 0.912} & {\color[HTML]{0000FF} 0.694} & {\color[HTML]{0000FF} 0.864} & {\underline{0.921}} & {\color[HTML]{0000FF} 0.871} & 0.516 & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.770}} & {\underline{0.932}} & {\color[HTML]{0000FF} 0.890} & {\color[HTML]{0000FF} 0.551} & {\color[HTML]{0000FF} 0.791} \\ 

\midrule
\midrule

\multicolumn{1}{c|}{Dataset} & \multicolumn{8}{c|}{Cora} & \multicolumn{8}{c}{Cora-A} \\ 
\midrule
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c|}{\scriptsize AP} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c}{\scriptsize AP} \\ 
\midrule
\multicolumn{1}{c|}{Test set} & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG \\ 
\midrule
\multicolumn{1}{c|}{Expansion} & 0.470 & 0.707 & 0.256 & \multicolumn{1}{c|}{0.478} & 0.637 & 0.764 & 0.454 & 0.618 & 0.690 & 0.842 & 0.434 & \multicolumn{1}{c|}{0.655} & 0.690 & 0.876 & 0.577 & 0.714 \\
\multicolumn{1}{c|}{NHP} & 0.943 & 0.641 & 0.472 & \multicolumn{1}{c|}{0.685} & 0.949 & 0.678 & 0.509 & 0.712 & 0.909 & 0.672 & 0.550 & \multicolumn{1}{c|}{0.710} & 0.925 & 0.720 & 0.585 & 0.743 \\
\multicolumn{1}{c|}{HyperSAGNN} & 0.617 & 0.527 & 0.494 & \multicolumn{1}{c|}{0.546} & 0.687 & 0.574 & 0.508 & 0.590 & 0.386 & 0.591 & 0.542 & \multicolumn{1}{c|}{0.506} & 0.532 & 0.643 & 0.545 & 0.573 \\
\multicolumn{1}{c|}{AHP} & {\underline{0.964}} & {\underline{0.860}} & {\underline{0.572}} & \multicolumn{1}{c|}{{\underline{0.799}}} & {\underline{0.961}} & {\underline{0.837}} & {\underline{0.552}} & {\underline{0.783}} & {\underline{0.958}} & {\underline{0.924}} & {\underline{0.782}} & \multicolumn{1}{c|}{{\underline{0.888}}} & {\underline{0.957}} & {\underline{0.898}} & {\underline{0.796}} & {\underline{0.884}} \\
\multicolumn{1}{c|}{{\method}} & {\color[HTML]{0000FF} 0.991} & {\color[HTML]{0000FF} 0.907} & {\color[HTML]{0000FF} 0.584} & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.827}} & {\color[HTML]{0000FF} 0.990} & {\color[HTML]{0000FF} 0.896} & {\color[HTML]{0000FF} 0.570} & {\color[HTML]{0000FF} 0.819} & {\color[HTML]{0000FF} 0.977} & {\color[HTML]{0000FF} 0.947} & {\color[HTML]{0000FF} 0.803} & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.909}} & {\color[HTML]{0000FF} 0.977} & {\color[HTML]{0000FF} 0.914} & {\color[HTML]{0000FF} 0.829} & {\color[HTML]{0000FF} 0.907} \\

\midrule
\midrule

\multicolumn{1}{c|}{Dataset} & \multicolumn{8}{c|}{DBLP} & \multicolumn{8}{c}{DBLP-A} \\ 
\midrule
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c|}{\scriptsize AP} & \multicolumn{4}{c|}{\scriptsize AUROC} & \multicolumn{4}{c}{\scriptsize AP} \\ 
\midrule
\multicolumn{1}{c|}{Test set} & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG & SNS & MNS & CNS & \multicolumn{1}{c|}{AVG} & SNS & MNS & CNS & AVG \\ 
\midrule
\multicolumn{1}{c|}{Expansion} & 0.645 & 0.801 & 0.366 & \multicolumn{1}{c|}{0.604} & 0.751 & {\color[HTML]{0000FF} 0.856} & 0.518 & 0.708 & 0.470 & 0.707 & 0.256 & \multicolumn{1}{c|}{0.478} & 0.637 & 0.764 & 0.454 & 0.618 \\
\multicolumn{1}{c|}{NHP} & 0.663 & 0.540 & 0.503 & \multicolumn{1}{c|}{0.569} & 0.608 & 0.523 & 0.501 & 0.544 & 0.943 & 0.641 & 0.472 & \multicolumn{1}{c|}{0.685} & 0.949 & 0.678 & 0.509 & 0.712 \\
\multicolumn{1}{c|}{HyperSAGNN} & 0.448 & 0.574 & 0.572 & \multicolumn{1}{c|}{0.531} & 0.562 & 0.602 & {\color[HTML]{0000FF} 0.586} & 0.583 & 0.617 & 0.527 & 0.494 & \multicolumn{1}{c|}{0.546} & 0.687 & 0.574 & 0.508 & 0.590 \\
\multicolumn{1}{c|}{AHP} & {\underline{0.946}} & {\underline{0.820}} & {\underline{0.568}} & \multicolumn{1}{c|}{{\underline{0.778}}} & {\underline{0.947}} & 0.815 & 0.561 & {\underline{0.774}} & {\underline{0.964}} & {\underline{0.860}} & {\underline{0.572}} & \multicolumn{1}{c|}{{\underline{0.799}}} & {\underline{0.961}} & {\underline{0.837}} & {\underline{0.552}} & {\underline{0.783}} \\
\multicolumn{1}{c|}{\method} & {\color[HTML]{0000FF} 0.958} & {\color[HTML]{0000FF} 0.839} & {\color[HTML]{0000FF} 0.591} & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.796}} & {\color[HTML]{0000FF} 0.958} & {\color[HTML]{0000FF} 0.826} & {\color[HTML]{0000FF} 0.573} & {\color[HTML]{0000FF} 0.786} & {\color[HTML]{0000FF} 0.991} & {\color[HTML]{0000FF} 0.907} & {\color[HTML]{0000FF} 0.584} & \multicolumn{1}{c|}{{\color[HTML]{0000FF} 0.827}} & {\color[HTML]{0000FF} 0.990} & {\color[HTML]{0000FF} 0.896} & {\color[HTML]{0000FF} 0.570} & {\color[HTML]{0000FF} 0.819} \\

\bottomrule
\end{tabular}
}
\end{table*}


==> tables/eq1-accuracy2.tex <==
\begin{table*}[t]
\centering

\caption{Hyperedge prediction accuracy: 
{\method} always outperforms all competing methods in both the average AP and AUROC across all datasets. (The \textbf{bold} and \underline{underlined} represents the best and the second-best results in each test set, respectively.)}\label{table:eval-accuracy}
% \vspace{-4mm}
\setlength\tabcolsep{1.6pt} % column space
\def\arraystretch{1.0} % row space

% \scriptsize
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|rrrr|rrrr|c|rrrr|rrrr|c|rrrr|rrrr}
\toprule

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{4}{c}{AUROC (\%)} & \multicolumn{4}{c|}{AP (\%)} & \multicolumn{1}{l|}{} & \multicolumn{4}{c}{AUROC (\%)} & \multicolumn{4}{c|}{AP (\%)} & \multicolumn{1}{l|}{} & \multicolumn{4}{c}{AUROC (\%)} & \multicolumn{4}{c}{AP (\%)} \\ 

\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){12-15} \cmidrule(lr){16-19} \cmidrule(lr){21-24} \cmidrule(lr){25-28} 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c}{AVG} & \multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c|}{AVG} & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c}{AVG} & 
\multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c|}{AVG} & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c}{AVG} & \multicolumn{1}{c}{SNS} & \multicolumn{1}{c}{MNS} & \multicolumn{1}{c}{CNS} & \multicolumn{1}{c}{AVG} \\

% \midrule
\midrule

Expansion & \multirow{5}{*}{\rotatebox{90}{Citeseer}} & 66.3 & 78.1 & 33.1 & 59.2 & 76.5 & 81.7 & 49.8 & 69.3 & \multirow{5}{*}{\rotatebox{90}{Pubmed}} & 52.0 & 73.0 & 24.1 & 49.7 & 67.5 & 75.5 & 44.0 & 62.3 &  \multirow{5}{*}{\rotatebox{90}{Cora}} & 47.0 & 70.7 & 25.6 & 47.8 & 63.7 & 76.4 & 45.4 & 61.8 \\ 
NHP & & \textbf{99.1} & 70.1 & 51.0 & 73.4 & \textbf{99.0} & 73.1 & 52.0 & 74.7 & & \textbf{97.3} & 69.4 & 52.4 & 73.0 & \textbf{97.3} & 65.6 & 51.3 & 71.4 & & 94.3 & 64.1 & 47.2 & 68.5 & 94.9 & 67.8 & 50.9 & 71.2\\ 
HyperSAGNN & & 54.0 & 41.0 & 47.3 & 47.4 & 62.7 & 45.5 & 49.7 & 52.6 & & 52.5 & 68.6 & \textbf{54.6} & 58.6 & 53.4 & 68.0 & \underline{52.9} & 58.1 & & 61.7 & 52.7 & 49.4 & 54.6 & 68.7 & 57.4 & 50.8 & 59.0\\ 
AHP & & 94.3 & \underline{88.1} & \underline{65.1} & \underline{82.5} & 95.2 & \underline{87.0} & \underline{66.0} & \underline{82.7} & & 91.7 & \underline{84.0} & \underline{53.3} & \underline{76.3} & 91.8 & \underline{83.4} & 52.6 & \underline{75.9} & & \underline{96.4} & \underline{86.0} & \underline{57.2} & \underline{79.9} & \underline{96.1} & \underline{83.7} & \underline{55.2} & \underline{78.3}\\

\textbf{\method} & & \underline{98.4} & \textbf{92.6} & \textbf{67.6} & \textbf{86.2} & \underline{98.5} & \textbf{91.2} & \textbf{69.4} & \textbf{86.4} & & \underline{92.1} & \textbf{87.1} & 51.6 & \textbf{77.0} & \underline{93.2} & \textbf{89.0} & \textbf{55.1} & \textbf{79.1} && \textbf{99.1} & \textbf{90.7} &  \textbf{58.4} & \textbf{82.7} & \textbf{99.0} & \textbf{89.6} &  \textbf{57.0} &  \textbf{81.9}  \\

% \cellcolor{gray!20}{\textbf{\method}} & & \cellcolor{gray!20}\underline{98.4} & \cellcolor{gray!20}\textbf{92.6} & \cellcolor{gray!20}\textbf{67.6} & \cellcolor{gray!20}\textbf{86.2} & \cellcolor{gray!20}\underline{98.5} & \cellcolor{gray!20}\textbf{91.2} & \cellcolor{gray!20}\textbf{69.4} & \cellcolor{gray!20}\textbf{86.4} & & \cellcolor{gray!20}\underline{92.1} & \cellcolor{gray!20}\textbf{87.1} & \cellcolor{gray!20}51.6 & \cellcolor{gray!20}\textbf{77.0} & \cellcolor{gray!20}\underline{93.2} & \cellcolor{gray!20}\textbf{89.0} & \cellcolor{gray!20}\textbf{55.1} & \cellcolor{gray!20}\textbf{79.1} && \cellcolor{gray!20} \textbf{99.1} & \cellcolor{gray!20} \textbf{90.7} & \cellcolor{gray!20} \textbf{58.4} & \cellcolor{gray!20} \textbf{82.7} & \cellcolor{gray!20} \textbf{99.0} & \cellcolor{gray!20} \textbf{89.6} & \cellcolor{gray!20} \textbf{57.0} & \cellcolor{gray!20} \textbf{81.9}  \\

\midrule
% \midrule
Expansion & \multirow{5}{*}{\rotatebox{90}{Cora-A}} & 69.0 & 84.2 & 43.4 & 65.5 & 69.0 & 87.6 & 57.7 & 71.4 
& \multirow{5}{*}{\rotatebox{90}{DBLP}} & 64.5 & 80.1 & 36.6 & 60.4 & 75.1 & \textbf{85.6} & 51.8 & 70.8 
& \multirow{5}{*}{\rotatebox{90}{DBLP-A}} & 63.4 & 82.6 & 35.0 & 60.3 & 73.0 & \textbf{85.2} & 51.2 & 69.8  \\ 
NHP & & 90.9 & 67.2 & 55.0 & 71.0 & 92.5 & 72.0 & 58.5 & 74.3  
& & 66.3 & 54.0 & 50.3 & 56.9 & 60.8 & 52.3 & 50.1 & 54.4 
& & \textbf{96.6} & 62.3 & 55.5 &\underline{ 71.5} & \textbf{96.5} & 60.4 & 53.4 & 70.1 \\ 

HyperSAGNN & & 38.6 & 59.1 & 54.2 & 50.6 & 53.2 & 64.3 & 54.5 & 57.3  
& & 44.8 & 57.4 & 57.2 & 53.1 & 56.2 & 60.2 & \textbf{58.6} & 58.3 
& & 54.8 & 79.1 & 56.3 & 63.4 & 68.6 & 80.5 & \textbf{55.2} & 68.1 \\ 

AHP & & \underline{95.8} & \underline{92.4} & \underline{78.2} & \underline{88.8} & \underline{95.7} & \underline{89.8} & \underline{79.6} & \underline{88.4} 
& & \underline{94.6} & \underline{82.0} & \underline{56.8} & \underline{77.8} & \underline{94.7} & 81.5 & 56.1 & \underline{77.4} 
& &\underline{ 91.6} &\underline{ 92.6} &\underline{ 66.8} &\textbf{83.7} &\underline{ 92.8} &\underline{ 92.8} &\underline{ 70.7} &\underline{ 85.4} \\ 

 \textbf{\method} & &  \textbf{97.7} &  \textbf{94.7} &  \textbf{80.3} &  \textbf{90.9} &  \textbf{97.7} &  \textbf{91.4} &  \textbf{82.9} &  \textbf{90.7} & &  \textbf{95.8} &  \textbf{83.9} &  \textbf{59.1} &  \textbf{79.6} &  \textbf{95.8} &  \underline{82.6} &  \underline{57.3} &  \textbf{78.6}  & & {91.3} &  \textbf{92.7} &  \textbf{67.1} &  \textbf{83.7} & {92.7} & \textbf{92.9} & \textbf{71.5} &  \textbf{85.7} \\


% \cellcolor{gray!20} \textbf{\method} 
% & & \cellcolor{gray!20} \textbf{97.7} & \cellcolor{gray!20} \textbf{94.7} & \cellcolor{gray!20} \textbf{80.3} & \cellcolor{gray!20} \textbf{90.9} & \cellcolor{gray!20} \textbf{97.7} & \cellcolor{gray!20} \textbf{91.4} & \cellcolor{gray!20} \textbf{82.9} & \cellcolor{gray!20} \textbf{90.7} 
% & & \cellcolor{gray!20} \textbf{95.8} & \cellcolor{gray!20} \textbf{83.9} & \cellcolor{gray!20} \textbf{59.1} & \cellcolor{gray!20} \textbf{79.6} & \cellcolor{gray!20} \textbf{95.8} & \cellcolor{gray!20} \underline{82.6} & \cellcolor{gray!20} \underline{57.3} & \cellcolor{gray!20} \textbf{78.6} 
% & & \cellcolor{gray!20}{91.3} & \cellcolor{gray!20} \textbf{92.7} & \cellcolor{gray!20} \textbf{67.1} & \cellcolor{gray!20} \textbf{83.7} & \cellcolor{gray!20}{92.7} & \cellcolor{gray!20}\textbf{92.9} & \cellcolor{gray!20}\textbf{71.5} & \cellcolor{gray!20} \textbf{85.7} \\



% \midrule

% Expansion &  \multirow{5}{*}{\rotatebox{90}{DBLP}} & 64.5 & 80.1 & 36.6 & 60.4 & 75.1 & \textbf{85.6} & 51.8 & 70.8 &  \multirow{5}{*}{\rotatebox{90}{DBLP-A}} & 47.0 & 70.7 & 25.6 & 47.8 & 63.7 & 76.4 & 45.4 & 61.8 \\ 
% NHP & & 66.3 & 54.0 & 50.3 & 56.9 & 60.8 & 52.3 & 50.1 & 54.4 & & 94.3 & 64.1 & 47.2 & 68.5 & 94.9 & 67.8 & 50.9 & 71.2 \\ 
% HyperSAGNN & & 44.8 & 57.4 & 57.2 & 53.1 & 56.2 & 60.2 & \textbf{58.6} & 58.3 & & 61.7 & 52.7 & 49.4 & 54.6 & 68.7 & 57.4 & 50.8 & 59.0 \\ 
% AHP & & \underline{94.6} & \underline{82.0} & \underline{56.8} & \underline{77.8} & \underline{94.7} & 81.5 & 56.1 & \underline{77.4} & & \underline{96.4} & \underline{86.0} & \underline{57.2} & \underline{79.9} & \underline{96.1} & \underline{83.7} & \underline{55.2} & \underline{78.3} \\
% \cellcolor{gray!20} \textbf{\method} & & \cellcolor{gray!20} \textbf{95.8} & \cellcolor{gray!20} \textbf{83.9} & \cellcolor{gray!20} \textbf{59.1} & \cellcolor{gray!20} \textbf{79.6} & \cellcolor{gray!20} \textbf{95.8} & \cellcolor{gray!20} \underline{82.6} & \cellcolor{gray!20} \underline{57.3} & \cellcolor{gray!20} \textbf{78.6} & & \cellcolor{gray!20} \textbf{99.1} & \cellcolor{gray!20} \textbf{90.7} & \cellcolor{gray!20} \textbf{58.4} & \cellcolor{gray!20} \textbf{82.7} & \cellcolor{gray!20} \textbf{99.0} & \cellcolor{gray!20} \textbf{89.6} & \cellcolor{gray!20} \textbf{57.0} & \cellcolor{gray!20} \textbf{81.9} \\

\bottomrule
\end{tabular}
}
\end{table*}



==> tables/eq2-ablation.tex <==
\begin{table*}[t]
\centering

\caption{Ablation study: Each of our proposed strategies is beneficial to improving the accuracy of {\method}.}\label{table:ablation}

\setlength\tabcolsep{2pt} % column space
\def\arraystretch{0.75} % row space

\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Citeseer}  & \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Cora-A} & \multicolumn{2}{c}{DBLP} & \multicolumn{2}{c}{DBLP-A} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
& {\scriptsize AUROC} & {\scriptsize AP} & {\scriptsize AUROC} & {\scriptsize AP} & {\scriptsize AUROC} & {\scriptsize AP} & {\scriptsize AUROC} & {\scriptsize AP} & {\scriptsize AUROC} & {\scriptsize AP} & {\scriptsize AUROC} & {\scriptsize AP} \\
\midrule\midrule
\textbf{{\method}} & \textbf{86.2} & \textbf{86.4} & \textbf{77.0} & \textbf{79.2} & \textbf{82.7} & \textbf{81.9} & \textbf{90.9} & \textbf{90.7} & \textbf{79.6} & \textbf{78.6} & \textbf{83.7} & \textbf{85.7} \\

\midrule

% \textbf{{\method}} w/o positive & 85.0 & 85.0 & \underline{76.9} & \underline{79.1} & 80.9 & 80.9 & 90.2 & 90.0 & 76.3 & 76.5 & \underline{83.0} & \underline{83.2} \\
%  Loss (\%) & \textcolor{red}{-1.33\%} & \textcolor{red}{-1.62\%} & \textcolor{red}{-0.11\%} & \textcolor{red}{-0.15\%} & \textcolor{red}{-2.22\%} & \textcolor{red}{-1.21\%} & \textcolor{red}{-0.72\%} & \textcolor{red}{-0.68\%} & \textcolor{red}{-4.15\%} & \textcolor{red}{-2.69\%} & \textcolor{red}{-0.84\%} & \textcolor{red}{-2.88\%} \\
w/o positive (\%) & 85.0 \textcolor{red}{(-1.33)} & 85.0 \textcolor{red}{(-1.62)} & \underline{76.9} \textcolor{red}{(-0.11)} & \underline{79.1} \textcolor{red}{(-0.15)} & 80.9 \textcolor{red}{(-2.22)} & 80.9 \textcolor{red}{(-1.21)} & 90.2 \textcolor{red}{(-0.72)} & 90.0 \textcolor{red}{(-0.68)} & 76.3 \textcolor{red}{(-4.15)} & 76.5 \textcolor{red}{(-2.69)} & \underline{83.0} \textcolor{red}{(-0.84)} & \underline{83.2} \textcolor{red}{(-2.88)} \\

\midrule

w/o enc-dec (\%) & \underline{85.7} \textcolor{red}{(-0.59)} & \underline{86.0} \textcolor{red}{(-0.41)} & 76.5 \textcolor{red}{(-0.53)} & 78.9 \textcolor{red}{(-0.24)} & \underline{81.9} \textcolor{red}{(-1.05)} & \underline{81.1} \textcolor{red}{(-0.87)} & \underline{89.8} \textcolor{red}{(-1.18)} & \underline{89.7} \textcolor{red}{(-1.03)} & \underline{75.2} \textcolor{red}{(-5.49)} & \underline{73.3} \textcolor{red}{(-6.68)} & 83.4 \textcolor{red}{(-0.28)} & 83.8 \textcolor{red}{(-2.18)} \\
% \textbf{{\method}} w/o Encoder-decoder & \underline{85.7} & \underline{86.0} & 76.5 & 78.9 & \underline{81.9} & \underline{81.1} & \underline{89.8} & \underline{89.7} & \underline{75.2} & \underline{73.3} & 83.4 & 83.8 \\
%  Loss (\%) & \textcolor{red}{-0.59\%} & \textcolor{red}{-0.41\%} & \textcolor{red}{-0.53\%} & \textcolor{red}{-0.24\%} & \textcolor{red}{-1.05\%} & \textcolor{red}{-0.87\%} & \textcolor{red}{-1.18\%} & \textcolor{red}{-1.03\%} & \textcolor{red}{-5.49\%} & \textcolor{red}{-6.68\%} & \textcolor{red}{-0.28\%} & \textcolor{red}{-2.18\%} \\

\midrule
w/o $L_{reg}$ (\%) & 82.4 \textcolor{red}{(-4.40)} & 82.9 \textcolor{red}{(-4.00)} & 76.8 \textcolor{red}{(-0.20)} & 77.1 \textcolor{red}{(-2.54)} & 78.5 \textcolor{red}{(-5.16)} & 78.2 \textcolor{red}{(-4.47)} & 89.5 \textcolor{red}{(-1.57)} & 89.4 \textcolor{red}{(-1.43)} & 72.7 \textcolor{red}{(-8.74)} & 72.4 \textcolor{red}{(-7.86)} & 70.9 \textcolor{red}{(-15.29)} & 61.6 \textcolor{red}{(-28.15)} \\

% \textbf{{\method}} w/o $L_{reg}$  & 82.4 & 82.9 & 76.8 & 77.1 & 78.5 & 78.2 & 89.5 & 89.4 & 72.7 & 72.4 & 70.9 & 61.6 \\
%  Loss (\%) & \textcolor{red}{-4.40\%} & \textcolor{red}{-4.00\%} & \textcolor{red}{-0.20\%} & \textcolor{red}{-2.54\%} & \textcolor{red}{-5.16\%} & \textcolor{red}{-4.47\%} & \textcolor{red}{-1.57\%} & \textcolor{red}{-1.43\%} & \textcolor{red}{-8.74\%} & \textcolor{red}{-7.86\%} & \textcolor{red}{-15.29\%} & \textcolor{red}{-28.15\%} \\
\bottomrule
\end{tabular}
}
\end{table*}

